Lost in Translation: A Study of Bugs Introduced by Large Language Models while Translating Code

Code translation aims to convert source code from one programming language (PL) to another. Given the promising abilities of large language models (LLMs) in code synthesis, researchers are exploring their potential to automate code translation. The prerequisite for advancing the state of LLM-based code translation is to understand their promises and limitations over existing techniques. To that end, we present a large-scale empirical study to investigate the ability of general LLMs and code LLMs for code translation across pairs of different languages, including C, C++, Go, Java, and Python. Our study, which involves the translation of 1,700 code samples from three benchmarks and two real-world projects, reveals that LLMs are yet to be reliably used to automate code translation -- with correct translations ranging from 2.1% to 47.3% for the studied LLMs. Further manual investigation of unsuccessful translations identifies 15 categories of translation bugs. We also compare LLM-based code translation with traditional non-LLM-based approaches. Our analysis shows that these two classes of techniques have their own strengths and weaknesses. Finally, insights from our study suggest that providing more context to LLMs during translation can help them produce better results. To that end, we propose a prompt-crafting approach based on the symptoms of erroneous translations; this improves the performance of LLM-based code translation by 5.5% on average. Our study is the first of its kind, in terms of scale and breadth, that provides insights into the current limitations of LLMs in code translation and opportunities for improving them. Our dataset -- consisting of 1,700 code samples in five PLs with 10K+ tests, 43K+ translated code, 1,748 manually labeled bugs, and 1,365 bug-fix pairs -- can help drive research in this area.

==> Sections/OldStructure/5-Fixing.tex <==
\section{RQ4: Fixing Bugs}

In this section, we assess the capability of GPT-4 in fixing unsuccessful translations. To help the model understand its mistake in unsuccessful translation, we include effect-specific feedback in prompts and re-query the model for fixing it. Our feedback includes \texttt{stderr} for compile/runtime error effects, and test input/output for functionally incorrect translations. In total, we perform two rounds of fixing, such that fixes are only applied on unsuccessful translations from the most recent attempt. Figure~\ref{fig:fixing} shows the performance of GPT-4 in fixing \codenet, \avatar, and \evalplus unsuccessful translations. In general, GPT-4 achieves almost perfect accuracy in translating \codenet snippets as these instances are very simple programs and only 1 test per instance. While majority of instances pass theirs tests, one major threat to validity of \codenet translations could be low quality of test data which does not expose potential bugs in translations. In contrast, GPT-4 performs significantly worse on \avatar and \evalplus due to (i) more complex instances, and (ii) more rigorous testing (x25 in \avatar and x16 in \evalplus). That is, when datasets have rigorous testing, the accuracy tends to be lower because a translation is considered successful if and only if it passes all tests.

Moreover, Figure~\ref{fig:fixing-effect} shows the distribution of unsuccessful translation effects after 3 attempts of translating. We observe vanilla prompting introduces a significant number of compilation (syntactical) and runtime errors in the generated translation. However, most of these errors are trivial to fix and as a result, first round of fixing (Fix-1) resolves most of these trivial mistakes and corrects the translation. Thus, the ratio of compilation and runtime errors decrease while the successful translations increase. In contrast, fixing functionally incorrect translations are not as trivial as fixing compile/runtime errors, hence, GPT-4 fails to fix most of functionally incorrect translations even after second attempt to fix unsuccessful translations.

Furthermore, we observe GPT-4 translates pairs which either belong to the same programming language paradigm (i.e., object-oriented), or have very close programming language concepts (i.e., static typing) very accurately. For instance, when translating any pair to Go, we observe the translation mostly suffers from compilation and runtime errors because its very different in design and concepts from other 4 languages. Precisely, in Go, a compilation error is raised if an imported library is not used in the program. In contrast, pairs like C-C++ are almost perfectly translated due to commonalities between these two languages.

\hl{include one big bar for codenet and avatar}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Resources/Figures/fix.pdf}
    \caption{Performance of GPT-4 in successfully translating code snippets with vanilla and effect-specific prompting.}
    \label{fig:fixing}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Resources/Figures/fixdist.pdf}
    \caption{Distribution of unsuccessful translations after vanilla prompting and 2 rounds of fixing.}
    \label{fig:fixing-effect}
\end{figure}


==> Sections/OldStructure/RQ2.tex <==
\section{RQ2: Bugs Introduced while Code Translation}

Based on the results from the previous RQ, we manually went through the bugs while using the best performing model for the code translation task. First, we build the taxonomy using open-coding approach~\cite{}, and then we label the bugs accordingly. 
\subsection{RQ2a: Taxonomy of Bugs}
\label{subsec:bugtypetaxonomy}
\input{Sections/4-Taxonomy}
\subsection{RQ2b: How Prevalent are These Bugs?}
\label{subsec:bugtypePrevalent}
\input{Sections/4-Challenges}

==> Sections/prev-section5.tex <==
\change{\section{Comparison with Existing Techniques}
\label{sec:comparison}

\input{Resources/Tables/comparison}

% To compare the existing code translation approaches with LLM, we performed a study to understand (a) the effectiveness of these two approaches (RQ3.1), and (b) the difference between the translation bug types (RQ3.2). Before discussing the RQs, we briefly discuss the setup of this experiment.

% \paragraph{Setup}
Next, we present our results for RQ3, in which we compare LLM-based code translation with existing code-translation techniques in terms of
their effectiveness (RQ3.1) and the differences in translation bugs (RQ3.2).
% It should be noted that certain tools did not lend themselves well to code translation, the reason for this will be elaborated upon below.

\textbf{Study Setup.}
We consider two categories of code-translation tools: transpilers (source-to-source compilers) and tools implementing learning-based techniques, such as statistical machine learning.
% (1) transpiler-based tools i.e., CxGo~\cite{c2go}, C2Rust~\cite{c2rust}, etc., and (b) statistical machine translation tools i.e., mppSMT~\cite{nguyen2015divide}, Tree2Tree~\cite{chen2018tree}, etc.

The tools in the first category leverage intermediate representation to translate code in one PL to another or enable cross-language translation by wrapping the code using various third-party libraries. We considered four tools in this category: CxGo~\cite{c2go} and C2Rust~\cite{c2rust}, which translate C to Go and Rust, respectively; and Sharpen~\cite{sharpen} and JavaToCSharp~\cite{java2csharp}, which translate Java to C\#. Of these, we could not use Sharpen and Java2Csharp. The available version of Sharpen (which is more than a decade old) failed in our attempts to use it and the tool is no longer maintained. For JavaToCSharp, we observed that none of the generated code instances compile and, in fact, require rewriting of library APIs (e.g., \texttt{\small System.in} (as confirmed by developers of the tool, who also said that JavaToCSharp is not built to perform full code migration).

%     \begin{itemize} [wide = 0pt]
%     \item \textbf{CxGo~\cite{c2go}.} \texttt{CxGO} uses a transpiler to translate C to Go. It uses \texttt{cc}---a C-compiler written in Go to transfrom the C code into a common abstract syntax tree (AST) to be able to represent both C and Go constructs collectively. This, in turn, is used to generate Golang code. We evaluated this tool on our C code snippets from \codenet and compared its performance with all our subject LLMs.
%     \item \textbf{C2Rust~\cite{c2rust}.} \texttt{C2Rust} is another transpiler which translates C to Rust by linking with the native clang compiler front end to parse C code and export its AST, which is then utilized by the Rust-implemented transpiler for translation. We evaluated this tool on our C code snippets from \codenet and compared its performance with all our subject LLMs.
%     \item \textbf{Sharpen~\cite{sharpen}.} This tool is a rule-based approach that heavily rely on third-party tools for translating Java to C\#. However, we are unable to use this tool as it is not actively maintained and resulted into many errors (last commit was a decade ago and uses significantly older Java version). Also the documentation page cannot be accessed anymore.

%     \item \textbf{JavaToCSharp~\cite{java2csharp}.} This tool also translates Java to C\#. We attempted to translated and noticed that this tool generates a C\# code which is not compilable, and requires major post-processing work (confirmed by developers of
% the tool) including rewriting libraries i.e., \texttt{\small System.in}. The developers of the tool confirmed JavaToCSharp is not meant to do full code migration.

% For instance, the \texttt{\small System} library exists both in Java and C\#, and when the translation involves \texttt{\small System.in}, the C\# compiler gets confused and cannot properly handle this case. Post-processing steps would need to re-write \texttt{\small System.in} into \texttt{java.lang.System.@in} in order to remove the ambiguity created during translation. The developers of the tool confirmed JavaToCSharp is not meant to do full code migration, and major post-processing is required to make the code compilable/executable. 
% Moreover, the translated code uses some Java compiled classes and requires linking of Java Development Tools (\texttt{\small jdt.jar}) with the C\# project through IKVM~\cite{ikvm} to work properly. This can become an issue as the translation tool could use the \texttt{\small .jar} file from a specific java version which might not be supported in the future.

% \rangeet{@Ali, Please fix the above paragraph. Justify each sentence. Q1. Why not compilable? Q2. What kind of post-processing needed? Q3. What did their developer confirm? Q4. Why requiring JDT with IKVM is an issue? Give proper justification. Now, it seems like the process requires much work but we got lazy and did not do that.} \ali{@Rangeet, I didn't get lazy to perform the post-processing. Reyhan mentioned that its better to talk about these limitations in the paper regarding alternative approaches. I justified some of your concerns in the text above.}}
    % \end{itemize}
    Statistical learning-based approaches. Another group of existing research employs statistical learning methods. We identified two tool in this category that translate Java to C\#. 
    % Examples include mppSMT~\cite{nguyen2015divide} and Tree2Tree~\cite{chen2018tree}, which have been used to translate Java to C\#. However, we were not able to perform a direct comparison of these tools with LLMs.
    \begin{itemize}[wide = 0pt]
        \item \textbf{mppSMT~\cite{nguyen2015divide}.} We attempted to access the tool artifacts by contacting the authors, but were unable to obtain any information.
 \item \textbf{Tree2Tree~\cite{chen2018tree}.} The complete artifacts of this tool are also not available. Further communication with the authors confirmed that the complete artifact was indeed missing. We attempted to train a similar model using their methodology but failed as the code and data are missing.
    \end{itemize}

\textbf{Dataset.} Based on the identified tools and ability to translate code, we use CodeNet and Avatar datasets for this experiment. For examples, we use the same one from C and Java that were selected previously.

\subsection{Comparison of Effectiveness}
\label{sect:effective}
In Table~\ref{table:comparison}, we depict the comparison of the traditional SE approaches with the effectiveness of the LLMs.

\textbf{C to Go.} When compared to LLMs, we found that CxGo outperforms all the open-source models with an accuracy of 62.25\%, but falls 10\% behind GPT-4. The biggest caveat is that executing code generated by CxGo requires specific libraries i.e., \texttt{stdio} for I/O operations instead of more generic \texttt{fmt} library. In terms of the effect of the incorrect translation, 46.7\% and 53.3\% are due to compilation and runtime errors. Whereas, for GPT-4, 76.3\%, 12.7\%, and 9.1\% errors are related to compilation, test, and runtime failures.

\textbf{C to Rust.}
Code written in C can be translated to Rust using this approach with significantly higher confidence (compared to GPT-4, produces 35\% more correct code). In case of GPT-4, most errors (50\%) are related to compilation errors. However, when we looked into these generated code closely, we found two major drawbacks. First, like most rule-based approaches, translated code lacks naturalness. As illustrated in Figure~\ref{}, when comparing the original C code, the GPT-4 translated version, and the C2Rust translation, it's noticeable that the GPT-4 translation is more natural and incorporates idiomatic expressions specific to the target language, rather than adapting C language functions to Rust (i.e. X from libc). Secondly, a notable issue with the C2Rust translation is the loss of safety guarantees, a concern not as prominent with other methods. 
\rangeet{@Rahul, put your analysis here}

%\textbf{Java to C\#.}
\subsection{Differences in Translation Bugs}
For understanding the differences in the translation bugs introduced by traditional SE and LLM-based approaches, we manually investigate them. We compare the code generated by LLM with the traditional approach.

\textbf{C to Go.}
In the case of GPT-4, most bugs (71.8\%) while translating C to Go are related to unused imports, variables, and other target language-specific violations, followed by incorrect input parsing (10.3\%). Whereas, with \texttt{CxGo} tool, the majority of the bugs are related to input parsing (26.7\%) and mismatch of behavior after replacing API call (26.7\%). In most cases, when the input parsing related API, i.e., \texttt{scanf} has been replaced by an API call that uses a custom library written specifically for the tool. Other errors include missing definitions of API in the custom library that has been called while translating the code.

\textbf{C to Rust.} While translating C code to Rust using GPT-4, most bugs are related to incorrect input parsing (38.1\%) and incorrect data types (17.9\%). Whereas, for \texttt{C2Rust} tool, there are very few bugs, and out of them majority are generated by the unused import lint checker, which is causing the code to stop compiling.
}



% \subsubsection{Rule-based Approaches}
% \change{There are two classes of rule-based approaches. One that leverages intermediate representation to translate code in one PL to another. Another one enables the cross language translation by wrapping the code using various third-party libraries. In this space, for language translation, there are several existing approaches i.e., CxGo~\cite{c2go}, C2Rust~\cite{c2rust}, Sharpen~\cite{sharpen}, JavaToCSharp~\cite{j2csharp}, etc. Based on those tools, we perform more experiments on C to Go, C to Rust, and Java to C\#. In Table~\ref{table:comparison}, we depict the results.}

% \change{\textbf{CxGo~\cite{c2go}.} This is a transpiler-based approach that converts code from C to Go. This project is well maintained and there is a broader community around this. When compared to LLMs, we found that CxGo outperforms all the open-source models with an accuracy of 62.25\%, but falls 10\% behind GPT-4. The biggest caveat is that executing code generated by CxGo requires specific libraries i.e., \texttt{stdio} for I/O operations instead of more generic \texttt{fmt} library.}

% \change{\textbf{C2Rust~\cite{c2rust}.} Code written in C can be translated to Rust using this approach with significantly higher confidence (compared to GPT-4, produces 35\% more correct code). However, when we looked into these generated code closely, we found two major drawbacks. First, like most rule-based approaches, translated code lacks naturalness. As illustrated in Figure~\ref{}, when comparing the original C code, the GPT-4 translated version, and the C2Rust translation, it's noticeable that the GPT-4 translation is more natural and incorporates idiomatic expressions specific to the target language, rather than adapting C language functions to Rust (i.e. X from libc). Secondly, a notable issue with the C2Rust translation is the loss of safety guarantees, a concern not as prominent with other methods. \rangeet{@Rahul, can you please fill the rest of the part.}}

% \change{\textbf{Sharpen~\cite{sharpen}.} This tool is a rule-based approach that heavily rely on third-party tools for translating Java to C\#. However, we are unable to use this tool as it is not actively maintained and resulted into many errors (last commit was a decade ago and uses significantly older Java version). Also the documentation page cannot be accessed anymore.}

% \change{\textbf{JavaToCSharp~\cite{java2csharp}.} This tool also translates Java to C\# and has an active community and maintenance. We translated all our Java code snippets from \codenet and \avatar using this tool to C\#. We noticed that this tool generates a C\# code which is not compilable, and requires major post-processing work (confirmed by developers of
% the tool). For instance, the \texttt{\small System} library exists both in Java and C\#, and when the translation involves \texttt{\small System.in}, the C\# compiler gets confused and cannot properly handle this case. Post-processing steps would need to re-write \texttt{\small System.in} into \texttt{java.lang.System.@in} in order to remove the ambiguity created during translation. The developers of the tool confirmed JavaToCSharp is not meant to do full code migration, and major post-processing is required to make the code compilable/executable. Moreover, the translated code uses some Java compiled classes and requires linking of Java Development Tools (\texttt{\small jdt.jar}) with the C\# project through IKVM~\cite{ikvm} to work properly. This can become an issue as the translation tool could use the \texttt{\small .jar} file from a specific java version which might not be supported in the future.
% \rangeet{@Ali, Please fix the above paragraph. Justify each sentence. Q1. Why not compilable? Q2. What kind of post-processing needed? Q3. What did their developer confirm? Q4. Why requiring JDT with IKVM is an issue? Give proper justification. Now, it seems like the process requires much work but we got lazy and did not do that.} \ali{@Rangeet, I didn't get lazy to perform the post-processing. Reyhan mentioned that its better to talk about these limitations in the paper regarding alternative approaches. I justified some of your concerns in the text above.}}


% \subsubsection{Statistical Learning-based Approaches}
% \change{
% Another group of existing research employs statistical learning methods. Examples include mppSMT~\cite{nguyen2015divide} and Tree2Tree~\cite{chen2018tree}, which have been used to translate Java to C\#. However, we were not able to perform a direct comparison of these tools with LLMs. We attempted to access the tool artifacts for mppSMT by contacting the authors, but were unable to obtain any information. Similarly, for Tree2Tree, the complete artifacts are not available, too. Further communication with the authors confirmed that the complete artifact was indeed missing. This also restricted us to train a similar model using their methodology as the code and data are missing.}

% \paragraph{mppSMT~\cite{nguyen2015divide}}

% \paragraph{Tree-to-Tree~\cite{chen2018tree}}

% \change{The second class of traditional translation techniques falls under the category of statistical and neural approaches. From this category, we attempted to evaluate the performance of mppSMT~\cite{nguyen2015divide} and Tree-to-tree~\cite{chen2018tree} which both translate Java to C\#. For the former, we reached out to the authors and inquired about the tool artifacts, and did not receive a response. As for Tree-to-tree, we asked the authors for either the pre-trained model to evaluate it on our dataset in a zero-shot manner, or their artifacts to pre-train a new model from scratch. In both cases, we were unsuccessful in acquiring complete artifacts from the authors. Tree2Tree uses Recurrent Neural Networks (RNNs) with Long Short-Term Memory (LSTM) to translate basic blocks from one programming language to another. We noticed that this tool only works when the input and output are in tree format, as opposed to raw source code (our evaluation dataset). Moreover, the evaluation metric used in this work does not involve test execution. It simply compares the translated tree with a ground truth and measures similarity without execution. This approach does not measure correct functional accuracy because a correct translation can be syntactically different from ground-truth, but semantically correct.}

%\subsubsection{Name something}


